Spin-Wave Optics in YIG by Ion-Beam Irradiation

We demonstrate direct focused ion beam (FIB) writing as an enabling technology for realizing spin-wave-optics devices. It is shown that ion-beam irradiation changes the characteristics of YIG films on a submicron scale in a highly controlled way, allowing to engineer the magnonic index of refraction adapted to desired applications. This technique does not physically remove material, and allows rapid fabrication of high-quality architectures of modified magnetization in magnonic media with minimal edge damage (compared to more common techniques such as etching or milling). By experimentally showing magnonic versions of a number of optical devices (lenses, gratings, Fourier-domain processors) we envision this technology as the gateway to building magnonic computing devices that rival their optical counterparts in their complexity and computational power.

==> Paper_Structure.tex <==
Paper Outline ...\\
This is space for discussion/open questions/annotations/remarks....\\
-  TEM images to supplementary section?\\
-  does the structure of sections make sense?\\
-  the color scale in the plot it always different (which makes sense!). Sometimes too much confusion/leave this out in some plots?\\
%
\section{Introduction}
%
- Optical metamaterials in optical computing\cite{wang2016optically}\\
- (future) spin wave based computing \cite{papp2020nanoscale}$^,$ \cite{chumak2019fundamentals}$^,$ \cite{klingler2015spin}\\
- magnon optics: key building blocks\cite{csaba2014spin}$^,$\cite{papp2016optically}$^,$ \cite{vogel2020optical}$^,$\cite{gross2020building}$->$ phase control  \cite{demidov2009control}\\
- attempts to alternate magnonic refractive index \cite{vogel2020optical}$^,$\cite{dobrovolskiy2019spin}\\
- attempts to physically structure YIG (magnonic wave guides) \cite{schlitz2019focused}\\
- magnonics confinements (boundaries, waveguides): local field changes, temperature maps, thickness variations, spin pumping (metals)... challenges of fab and patterning: ion etching, milling \cite{schlitz2019focused}$^,$\cite{collet2017spin}\\
- YIG as an insulating substrate: excess surface charge \cite{ruane2018controlling}\\
- Particularly: Spin Wave Lenses \cite{whitehead2018luneburg}$^,$\cite{toedt2016design}$^,$\cite{dai2020focusing}\\
- graded index magnonics \cite{davies2015towards}
%
%%% METHODS %%%
\section{Ion Beam Engineering of the Magnetic Properties in YIG}
- purpose: spatial modification of yig 
- Ga FIB in 100 nm 
- Basically explaining the experimental platform from the presentations...
\subsection{FIB Impact on Magnetic Properties}
- Meff and damping modification 
- \\
- \\
\subsection{Spin Wave Steering via Ion Dose}
- \\
- \\
- \\
%%% Results %%%
\section{Optically Inspired Magnonic Elements Based on Distinct Irradiation Effects}
- \\
- \\
- \\
\subsection{Increasing the Effective Magnetization to Tune the Relative Refractive Index}
- \\
- \\
- \\
\subsection{Locally Inhibited Spin Wave Propagation in Analogy to YIG Etching}
- \\
- \\
- \\
\subsection{Exploring the Applicability of FIB Manipulation}- \\
- \\
- \\
%
\section{Discussion}
- \\
- \\
- \\
\section*{Conclusion}
